Large Language Model-Powered Smart Contract Vulnerability Detection: New Perspectives

This paper provides a systematic analysis of the opportunities, challenges, and potential solutions of harnessing Large Language Models (LLMs) such as GPT-4 to dig out vulnerabilities within smart contracts based on our ongoing research. For the task of smart contract vulnerability detection, achieving practical usability hinges on identifying as many true vulnerabilities as possible while minimizing the number of false positives. Nonetheless, our empirical study reveals contradictory yet interesting findings: generating more answers with higher randomness largely boosts the likelihood of producing a correct answer but inevitably leads to a higher number of false positives. To mitigate this tension, we propose an adversarial framework dubbed GPTLens that breaks the conventional one-stage detection into two synergistic stages $-$ generation and discrimination, for progressive detection and refinement, wherein the LLM plays dual roles, i.e., auditor and critic, respectively. The goal of auditor is to yield a broad spectrum of vulnerabilities with the hope of encompassing the correct answer, whereas the goal of critic that evaluates the validity of identified vulnerabilities is to minimize the number of false positives. Experimental results and illustrative examples demonstrate that auditor and critic work together harmoniously to yield pronounced improvements over the conventional one-stage detection. GPTLens is intuitive, strategic, and entirely LLM-driven without relying on specialist expertise in smart contracts, showcasing its methodical generality and potential to detect a broad spectrum of vulnerabilities. Our code is available at: https://github.com/git-disl/GPTLens.

==> TPS23 <==
\begin{thebibliography}{10}

\bibitem{gpt3temp2021}
AlgoWriting.
\newblock A simple guide to setting the gpt-3 temperature, 2020.
\newblock \url{https://algowriting.medium.com/gpt-3-temperature-setting-101-41200ff0d0be}.

\bibitem{anthropic2022claude}
Anthropic.
\newblock Introducing claude.
\newblock Anthropic Blog, 2022.
\newblock \url{https://www.anthropic.com/index/introducing-claude}.

\bibitem{brent2020ethainter}
L.~Brent, N.~Grech, S.~Lagouvardos, B.~Scholz, and Y.~Smaragdakis.
\newblock Ethainter: a smart contract security analyzer for composite vulnerabilities.
\newblock In {\em Proceedings of the 41st ACM SIGPLAN Conference on Programming Language Design and Implementation}, pages 454--469, 2020.

\bibitem{brent2018vandal}
L.~Brent, A.~Jurisevic, M.~Kong, E.~Liu, F.~Gauthier, V.~Gramoli, R.~Holz, and B.~Scholz.
\newblock Vandal: A scalable security analysis framework for smart contracts.
\newblock {\em arXiv preprint arXiv:1809.03981}, 2018.

\bibitem{gpt3}
T.~Brown, B.~Mann, N.~Ryder, M.~Subbiah, J.~D. Kaplan, P.~Dhariwal, A.~Neelakantan, P.~Shyam, G.~Sastry, A.~Askell, et~al.
\newblock Language models are few-shot learners.
\newblock {\em Advances in neural information processing systems}, 33:1877--1901, 2020.

\bibitem{brown2020language}
T.~Brown, B.~Mann, N.~Ryder, M.~Subbiah, J.~D. Kaplan, P.~Dhariwal, A.~Neelakantan, P.~Shyam, G.~Sastry, A.~Askell, et~al.
\newblock Language models are few-shot learners.
\newblock {\em Advances in neural information processing systems}, 33:1877--1901, 2020.

\bibitem{cao2022gift}
Y.~Cao, S.~Hu, Y.~Gong, Z.~Li, Y.~Yang, Q.~Liu, and S.~Ji.
\newblock Gift: Graph-guided feature transfer for cold-start video click-through rate prediction.
\newblock In {\em Proceedings of the 31st ACM International Conference on Information \& Knowledge Management}, pages 2964--2973, 2022.

\bibitem{chen2023chatgpt}
C.~Chen, J.~Su, J.~Chen, Y.~Wang, T.~Bi, Y.~Wang, X.~Lin, T.~Chen, and Z.~Zheng.
\newblock When chatgpt meets smart contract vulnerability detection: How far are we?
\newblock {\em arXiv preprint arXiv:2309.05520}, 2023.

\bibitem{codex}
M.~Chen, J.~Tworek, H.~Jun, Q.~Yuan, H.~P. d.~O. Pinto, J.~Kaplan, H.~Edwards, Y.~Burda, N.~Joseph, G.~Brockman, et~al.
\newblock Evaluating large language models trained on code.
\newblock {\em arXiv preprint arXiv:2107.03374}, 2021.

\bibitem{david2023you}
I.~David, L.~Zhou, K.~Qin, D.~Song, L.~Cavallaro, and A.~Gervais.
\newblock Do you still need a manual smart contract audit?
\newblock {\em arXiv preprint arXiv:2306.12338}, 2023.

\bibitem{feist2019slither}
J.~Feist, G.~Grieco, and A.~Groce.
\newblock Slither: a static analysis framework for smart contracts.
\newblock In {\em 2019 IEEE/ACM 2nd International Workshop on Emerging Trends in Software Engineering for Blockchain (WETSEB)}, pages 8--15. IEEE, 2019.

\bibitem{GAN}
I.~Goodfellow, J.~Pouget-Abadie, M.~Mirza, B.~Xu, D.~Warde-Farley, S.~Ozair, A.~Courville, and Y.~Bengio.
\newblock Generative adversarial nets.
\newblock {\em Advances in neural information processing systems}, 27, 2014.

\bibitem{grieco2020echidna}
G.~Grieco, W.~Song, A.~Cygan, J.~Feist, and A.~Groce.
\newblock Echidna: effective, usable, and fast fuzzing for smart contracts.
\newblock In {\em Proceedings of the 29th ACM SIGSOFT International Symposium on Software Testing and Analysis}, pages 557--560, 2020.

\bibitem{heller1999catch}
J.~Heller.
\newblock {\em Catch-22: a novel}, volume~4.
\newblock Simon and Schuster, 1999.

\bibitem{hou2023large}
X.~Hou, Y.~Zhao, Y.~Liu, Z.~Yang, K.~Wang, L.~Li, X.~Luo, D.~Lo, J.~Grundy, and H.~Wang.
\newblock Large language models for software engineering: A systematic literature review.
\newblock {\em arXiv preprint arXiv:2308.10620}, 2023.

\bibitem{hu2023bert4eth}
S.~Hu, Z.~Zhang, B.~Luo, S.~Lu, B.~He, and L.~Liu.
\newblock Bert4eth: A pre-trained transformer for ethereum fraud detection.
\newblock In {\em Proceedings of the ACM Web Conference 2023}, pages 2189--2197, 2023.

\bibitem{jeon2021smartcondetect}
S.~Jeon, G.~Lee, H.~Kim, and S.~S. Woo.
\newblock Smartcondetect: Highly accurate smart contract code vulnerability detection mechanism using bert.
\newblock In {\em KDD Workshop on Programming Language Processing}, 2021.

\bibitem{jiang2018contractfuzzer}
B.~Jiang, Y.~Liu, and W.~K. Chan.
\newblock Contractfuzzer: Fuzzing smart contracts for vulnerability detection.
\newblock In {\em Proceedings of the 33rd ACM/IEEE International Conference on Automated Software Engineering}, pages 259--269, 2018.

\bibitem{kalra2018zeus}
S.~Kalra, S.~Goel, M.~Dhawan, and S.~Sharma.
\newblock Zeus: analyzing safety of smart contracts.
\newblock In {\em Ndss}, pages 1--12, 2018.

\bibitem{alphacode}
Y.~Li, D.~Choi, J.~Chung, N.~Kushman, J.~Schrittwieser, R.~Leblond, T.~Eccles, J.~Keeling, F.~Gimeno, A.~Dal~Lago, et~al.
\newblock Competition-level code generation with alphacode.
\newblock {\em Science}, 378(6624):1092--1097, 2022.

\bibitem{liao2022smartdagger}
Z.~Liao, Z.~Zheng, X.~Chen, and Y.~Nan.
\newblock Smartdagger: a bytecode-based static analysis approach for detecting cross-contract vulnerability.
\newblock In {\em Proceedings of the 31st ACM SIGSOFT International Symposium on Software Testing and Analysis}, pages 752--764, 2022.

\bibitem{liu2021smart}
Z.~Liu, P.~Qian, X.~Wang, L.~Zhu, Q.~He, and S.~Ji.
\newblock Smart contract vulnerability detection: from pure neural network to interpretable graph feature and expert pattern fusion.
\newblock {\em arXiv preprint arXiv:2106.09282}, 2021.

\bibitem{liu2021combining}
Z.~Liu, P.~Qian, X.~Wang, Y.~Zhuang, L.~Qiu, and X.~Wang.
\newblock Combining graph neural networks with expert knowledge for smart contract vulnerability detection.
\newblock {\em IEEE Transactions on Knowledge and Data Engineering}, 2021.

\bibitem{mossberg2019manticore}
M.~Mossberg, F.~Manzano, E.~Hennenfent, A.~Groce, G.~Grieco, J.~Feist, T.~Brunson, and A.~Dinaburg.
\newblock Manticore: A user-friendly symbolic execution framework for binaries and smart contracts.
\newblock In {\em 2019 34th IEEE/ACM International Conference on Automated Software Engineering (ASE)}, pages 1186--1189. IEEE, 2019.

\bibitem{mythril2023}
Mythril.
\newblock \url{https://github.com/Consensys/mythril}.

\bibitem{openai2023gpt4}
OpenAI.
\newblock Gpt-4 technical report, 2023.
\newblock \url{https://arxiv.org/abs/2303.08774}.

\bibitem{park2023generative}
J.~S. Park, J.~C. O'Brien, C.~J. Cai, M.~R. Morris, P.~Liang, and M.~S. Bernstein.
\newblock Generative agents: Interactive simulacra of human behavior.
\newblock {\em arXiv preprint arXiv:2304.03442}, 2023.

\bibitem{paul2023automated}
R.~Paul, M.~M. Hossain, M.~Hasan, and A.~Iqbal.
\newblock Automated program repair based on code review: How do pre-trained transformer models perform?
\newblock {\em arXiv preprint arXiv:2304.07840}, 2023.

\bibitem{verx}
A.~Permenev, D.~Dimitrov, P.~Tsankov, D.~Drachsler-Cohen, and M.~Vechev.
\newblock Verx: Safety verification of smart contracts.
\newblock In {\em 2020 IEEE symposium on security and privacy (SP)}, pages 1661--1677. IEEE, 2020.

\bibitem{qian2023communicative}
C.~Qian, X.~Cong, C.~Yang, W.~Chen, Y.~Su, J.~Xu, Z.~Liu, and M.~Sun.
\newblock Communicative agents for software development.
\newblock {\em arXiv preprint arXiv:2307.07924}, 2023.

\bibitem{qian2020towards}
P.~Qian, Z.~Liu, Q.~He, R.~Zimmermann, and X.~Wang.
\newblock Towards automated reentrancy detection for smart contracts based on sequential models.
\newblock {\em IEEE Access}, 8:19685--19695, 2020.

\bibitem{qian2023cross}
P.~Qian, Z.~Liu, Y.~Yin, and Q.~He.
\newblock Cross-modality mutual learning for enhancing smart contract vulnerability detection on bytecode.
\newblock In {\em Proceedings of the ACM Web Conference 2023}, pages 2220--2229, 2023.

\bibitem{radford2015unsupervised}
A.~Radford, L.~Metz, and S.~Chintala.
\newblock Unsupervised representation learning with deep convolutional generative adversarial networks.
\newblock {\em arXiv preprint arXiv:1511.06434}, 2015.

\bibitem{schick2023toolformer}
T.~Schick, J.~Dwivedi-Yu, R.~Dess{\`\i}, R.~Raileanu, M.~Lomeli, L.~Zettlemoyer, N.~Cancedda, and T.~Scialom.
\newblock Toolformer: Language models can teach themselves to use tools.
\newblock {\em arXiv preprint arXiv:2302.04761}, 2023.

\bibitem{sendner2023smarter}
C.~Sendner, H.~Chen, H.~Fereidooni, L.~Petzi, J.~K{\"o}nig, J.~Stang, A.~Dmitrienko, A.-R. Sadeghi, and F.~Koushanfar.
\newblock Smarter contracts: Detecting vulnerabilities in smart contracts with deep transfer learning.
\newblock In {\em NDSS}, 2023.

\bibitem{shen2022benchmarking}
D.~Shen, X.~Chen, C.~Wang, K.~Sen, and D.~Song.
\newblock Benchmarking language models for code syntax understanding.
\newblock {\em arXiv preprint arXiv:2210.14473}, 2022.

\bibitem{verismart}
S.~So, M.~Lee, J.~Park, H.~Lee, and H.~Oh.
\newblock Verismart: A highly precise safety verifier for ethereum smart contracts.
\newblock In {\em 2020 IEEE Symposium on Security and Privacy (SP)}, pages 1678--1694. IEEE, 2020.

\bibitem{sun2023assbert}
X.~Sun, L.~Tu, J.~Zhang, J.~Cai, B.~Li, and Y.~Wang.
\newblock Assbert: Active and semi-supervised bert for smart contract vulnerability detection.
\newblock {\em Journal of Information Security and Applications}, 73:103423, 2023.

\bibitem{sun2021attention}
Y.~Sun and L.~Gu.
\newblock Attention-based machine learning model for smart contract vulnerability detection.
\newblock In {\em Journal of physics: conference series}, volume 1820, page 012004. IOP Publishing, 2021.

\bibitem{gptscan}
Y.~Sun, D.~Wu, Y.~Xue, H.~Liu, H.~Wang, Z.~Xu, X.~Xie, and Y.~Liu.
\newblock When gpt meets program analysis: Towards intelligent detection of smart contract logic vulnerabilities in gptscan.
\newblock {\em arXiv preprint arXiv:2308.03314}, 2023.

\bibitem{tann2018towards}
W.~J.-W. Tann, X.~J. Han, S.~S. Gupta, and Y.-S. Ong.
\newblock Towards safer smart contracts: A sequence learning approach to detecting security threats.
\newblock {\em arXiv preprint arXiv:1811.06632}, 2018.

\bibitem{thapa2022transformer}
C.~Thapa, S.~I. Jang, M.~E. Ahmed, S.~Camtepe, J.~Pieprzyk, and S.~Nepal.
\newblock Transformer-based language models for software vulnerability detection.
\newblock In {\em Proceedings of the 38th Annual Computer Security Applications Conference}, pages 481--496, 2022.

\bibitem{touvron2023llama}
H.~Touvron, T.~Lavril, G.~Izacard, X.~Martinet, M.-A. Lachaux, T.~Lacroix, B.~Rozi{\`e}re, N.~Goyal, E.~Hambro, F.~Azhar, et~al.
\newblock Llama: Open and efficient foundation language models.
\newblock {\em arXiv preprint arXiv:2302.13971}, 2023.

\bibitem{tsankov2018securify}
P.~Tsankov, A.~Dan, D.~Drachsler-Cohen, A.~Gervais, F.~Buenzli, and M.~Vechev.
\newblock Securify: Practical security analysis of smart contracts.
\newblock In {\em Proceedings of the 2018 ACM SIGSAC conference on computer and communications security}, pages 67--82, 2018.

\bibitem{cve}
N.~vulnerability database.
\newblock Common vulnerabilities and exposures (cves).
\newblock \url{https://cve.mitre.org/index.html}.

\bibitem{wang2023codet5+}
Y.~Wang, H.~Le, A.~D. Gotmare, N.~D. Bui, J.~Li, and S.~C. Hoi.
\newblock Codet5+: Open code large language models for code understanding and generation.
\newblock {\em arXiv preprint arXiv:2305.07922}, 2023.

\bibitem{chain-of-thought}
J.~Wei, X.~Wang, D.~Schuurmans, M.~Bosma, F.~Xia, E.~Chi, Q.~V. Le, D.~Zhou, et~al.
\newblock Chain-of-thought prompting elicits reasoning in large language models.
\newblock {\em Advances in Neural Information Processing Systems}, 35:24824--24837, 2022.

\bibitem{dasp10}
D.~Wong and M.~Hemmel.
\newblock Decentralized application security project top 10 of 2018, 2018.

\bibitem{wu2023effective}
Y.~Wu, N.~Jiang, H.~V. Pham, T.~Lutellier, J.~Davis, L.~Tan, P.~Babkin, and S.~Shah.
\newblock How effective are neural networks for fixing security vulnerabilities.
\newblock {\em arXiv preprint arXiv:2305.18607}, 2023.

\bibitem{wustholz2020harvey}
V.~W{\"u}stholz and M.~Christakis.
\newblock Harvey: A greybox fuzzer for smart contracts.
\newblock In {\em Proceedings of the 28th ACM Joint Meeting on European Software Engineering Conference and Symposium on the Foundations of Software Engineering}, pages 1398--1409, 2020.

\bibitem{xi2023rise}
Z.~Xi, W.~Chen, X.~Guo, W.~He, Y.~Ding, B.~Hong, M.~Zhang, J.~Wang, S.~Jin, E.~Zhou, et~al.
\newblock The rise and potential of large language model based agents: A survey.
\newblock {\em arXiv preprint arXiv:2309.07864}, 2023.

\bibitem{xia2023automated}
C.~S. Xia, Y.~Wei, and L.~Zhang.
\newblock Automated program repair in the era of large pre-trained language models.
\newblock In {\em Proceedings of the 45th International Conference on Software Engineering (ICSE 2023). Association for Computing Machinery}, 2023.

\bibitem{xue2022xfuzz}
Y.~Xue, J.~Ye, W.~Zhang, J.~Sun, L.~Ma, H.~Wang, and J.~Zhao.
\newblock xfuzz: Machine learning guided cross-contract fuzzing.
\newblock {\em IEEE Transactions on Dependable and Secure Computing}, 2022.

\bibitem{yao2023tree}
S.~Yao, D.~Yu, J.~Zhao, I.~Shafran, T.~L. Griffiths, Y.~Cao, and K.~Narasimhan.
\newblock Tree of thoughts: Deliberate problem solving with large language models.
\newblock {\em arXiv preprint arXiv:2305.10601}, 2023.

\bibitem{zhang2019mpro}
W.~Zhang, S.~Banescu, L.~Pasos, S.~Stewart, and V.~Ganesh.
\newblock Mpro: Combining static and symbolic analysis for scalable testing of smart contract.
\newblock In {\em 2019 IEEE 30th International Symposium on Software Reliability Engineering (ISSRE)}, pages 456--462. IEEE, 2019.

\bibitem{zhang2023cumulative}
Y.~Zhang, J.~Yang, Y.~Yuan, and A.~C.-C. Yao.
\newblock Cumulative reasoning with large language models.
\newblock {\em arXiv preprint arXiv:2308.04371}, 2023.

\bibitem{zhang2023demystifying}
Z.~Zhang, B.~Zhang, W.~Xu, and Z.~Lin.
\newblock Demystifying exploitable bugs in smart contracts.
\newblock ICSE, 2023.

\bibitem{zhao2023survey}
W.~X. Zhao, K.~Zhou, J.~Li, T.~Tang, X.~Wang, Y.~Hou, Y.~Min, B.~Zhang, J.~Zhang, Z.~Dong, et~al.
\newblock A survey of large language models.
\newblock {\em arXiv preprint arXiv:2303.18223}, 2023.

\bibitem{zhou2023sok}
L.~Zhou, X.~Xiong, J.~Ernstberger, S.~Chaliasos, Z.~Wang, Y.~Wang, K.~Qin, R.~Wattenhofer, D.~Song, and A.~Gervais.
\newblock Sok: Decentralized finance (defi) attacks.
\newblock In {\em 2023 IEEE Symposium on Security and Privacy (SP)}, pages 2444--2461. IEEE, 2023.

\bibitem{zhuang2021smart}
Y.~Zhuang, Z.~Liu, P.~Qian, Q.~Liu, X.~Wang, and Q.~He.
\newblock Smart contract vulnerability detection using graph neural networks.
\newblock In {\em Proceedings of the Twenty-Ninth International Conference on International Joint Conferences on Artificial Intelligence}, pages 3283--3290, 2021.

\end{thebibliography}

